A class of static spherically symmetric solutions in $f(T)$-gravity

We study a class of static spherically symmetric vacuum solutions in modified teleparallel gravity solving the field equations for a specific model Ansatz, requiring the torsion scalar $T$ to be constant. We discuss the models falling in this class. After some general considerations, we provide and investigate local solutions in the form of black holes and traversable wormholes as well as configurations that can match the anomalous rotation curves of galaxies.

==> Bib.tex <==

%%%%%%%%%%%%%%%% TEGR %%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\bibitem{BeltranJimenez:2019esp}
J.~Beltr\'an Jim\'enez, L.~Heisenberg and T.~S.~Koivisto,
%``The Geometrical Trinity of Gravity,''
Universe \textbf{5}, no.7, 173 (2019)
%doi:10.3390/universe5070173
%[arXiv:1903.06830 [hep-th]].
%178 citations counted in INSPIRE as of 18 Jul 2022.

\bibitem{Springer}
R.~Aldrovandi and J.~G.~Pereira,
%Teleparallel Gravity
, Vol. 173 (Springer, Dordrecht, 2013).


\bibitem{Maluf:2013gaa}
J.~W.~Maluf,
%``The teleparallel equivalent of general relativity,''
Annalen Phys. \textbf{525}, 339-357 (2013)
doi:10.1002/andp.201200272
[arXiv:1303.3897 [gr-qc]].
%275 citations counted in INSPIRE as of 18 Jul 2022




\bibitem{moltoaltro}
K. F. Dialektopoulos, T. S. Koivisto and S. Capozziello,
Eur. Phys. J. C 79, no.7, 606 (2019);
 B. J. Barros, T. Barreiro, T. Koivisto and N. J. Nunes,
Phys. Dark Univ. 30, 100616 (2020);
J. Beltran Jimenez, L. Heisenberg,
 T. S. Koivisto and
S. Pekar, Phys. Rev. D 101, no.10, 103507 (2020);
F. Bajardi, D. Vernieri and S. Capozziello, Eur. Phys. J.
Plus 135, no.11, 912 (2020);
I. Ayuso, R. Lazkoz and V. Salzano, Phys. Rev. D 103,
no.6, 063505 (2021);
K. Flathmann and M. Hohmann, Phys. Rev. D 103, no.4,
044030 (2021);
 N. Frusciante, Phys. Rev. D 103, no.4, 044021 (2021);  W. Khyllep, A. Paliathanasis and J. Dutta, Phys. Rev.
D 103, no.10, 103521 (2021);
 F. D`Ambrosio, M. Garg and L. Heisenberg, Phys. Lett.
B 811, 135970 (2020).

%%%%%%%%%%%%%%%% STEGR %%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%
\bibitem{Nester:1998mp}
J.~M.~Nester and H.~J.~Yo,
%``Symmetric teleparallel general relativity,''
Chin. J. Phys. \textbf{37}, 113 (1999)
[arXiv:gr-qc/9809049 [gr-qc]].
%170 citations counted in INSPIRE as of 18 Jul 2022

%\cite{}
\bibitem{Adak:2004uh}
M.~Adak and O.~Sert,
%``A Solution to symmetric teleparallel gravity,''
Turk. J. Phys. \textbf{29}, 1-7 (2005)
[arXiv:gr-qc/0412007 [gr-qc]].
%27 citations counted in INSPIRE as of 18 Jul 2022


%\cite{}
\bibitem{Adak:2005cd}
M.~Adak, M.~Kalay and O.~Sert,
%``Lagrange formulation of the symmetric teleparallel gravity,''
Int. J. Mod. Phys. D \textbf{15}, 619-634 (2006)
doi:10.1142/S0218271806008474
[arXiv:gr-qc/0505025 [gr-qc]].
%50 citations counted in INSPIRE as of 18 Jul 2022


%\cite{}
\bibitem{Adak:2008gd}
M.~Adak, \"O.~Sert, M.~Kalay and M.~Sari,
%``Symmetric Teleparallel Gravity: Some exact solutions and spinor couplings,''
Int. J. Mod. Phys. A \textbf{28}, 1350167 (2013)
doi:10.1142/S0217751X13501674
[arXiv:0810.2388 [gr-qc]].
%39 citations counted in INSPIRE as of 18 Jul 2022

%\cite{}
\bibitem{Mol:2014ooa}
I.~Mol,
%``The Non-Metricity Formulation of General Relativity,''
Adv. Appl. Clifford Algebras \textbf{27}, no.3, 2607-2638 (2017)
doi:10.1007/s00006-016-0749-8
[arXiv:1406.0737 [gr-qc]].
%30 citations counted in INSPIRE as of 18 Jul 2022


%\cite{}
\bibitem{BeltranJimenez:2017tkd}
J.~Beltr\'an Jim\'enez, L.~Heisenberg and T.~Koivisto,
%``Coincident General Relativity,''
Phys. Rev. D \textbf{98}, no.4, 044048 (2018)
doi:10.1103/PhysRevD.98.044048
[arXiv:1710.03116 [gr-qc]].
%194 citations counted in INSPIRE as of 18 Jul 2022

%\cite{}
\bibitem{BeltranJimenez:2018vdo}
J.~Beltr\'an Jim\'enez, L.~Heisenberg and T.~S.~Koivisto,
%``Teleparallel Palatini theories,''
JCAP \textbf{08}, 039 (2018)
doi:10.1088/1475-7516/2018/08/039
[arXiv:1803.10185 [gr-qc]].
%101 citations counted in INSPIRE as of 18 Jul 2022

%\cite{}
\bibitem{Gakis:2019rdd}
V.~Gakis, M.~Kr\v{s}\v{s}\'ak, J.~Levi Said and E.~N.~Saridakis,
%``Conformal gravity and transformations in the symmetric teleparallel framework,''
Phys. Rev. D \textbf{101}, no.6, 064024 (2020)
doi:10.1103/PhysRevD.101.064024
[arXiv:1908.05741 [gr-qc]].
%18 citations counted in INSPIRE as of 18 Jul 2022



%\cite{}
\bibitem{Jarv:2018bgs}
L.~J\"arv, M.~R\"unkla, M.~Saal and O.~Vilson,
%``Nonmetricity formulation of general relativity and its scalar-tensor extension,''
Phys. Rev. D \textbf{97}, no.12, 124025 (2018)
doi:10.1103/PhysRevD.97.124025
[arXiv:1802.00492 [gr-qc]].
%81 citations counted in INSPIRE as of 18 Jul 2022



\bibitem{Capozziello}
S.~Capozziello, V.~De Falco and C.~Ferrara,
%``Comparing Equivalent Gravities: common features and differences,''
[arXiv:2208.03011 [gr-qc]].
%0 citations counted in INSPIRE as of 10 Aug 2022


%\cite{}
\bibitem{Heisenberg:2018vsk}
L.~Heisenberg,
%``A systematic approach to generalisations of General Relativity and their cosmological implications,''
Phys. Rept. \textbf{796} (2019), 1-113
%doi:10.1016/j.physrep.2018.11.006
%[arXiv:1807.01725 [gr-qc]].
%213 citations counted in INSPIRE as of 01 Sep 2022



%%%%%%%%%%%%% f(R) %%%%%%%%%%%%%%%%%%%%%%%%%%


%\cite{}
\bibitem{DeFelice:2010aj}
A.~De Felice and S.~Tsujikawa,
%``f(R) theories,''
Living Rev. Rel. \textbf{13}, 3 (2010)
doi:10.12942/lrr-2010-3
[arXiv:1002.4928 [gr-qc]].
%2667 citations counted in INSPIRE as of 18 Jul 2022


%
\bibitem{Sotiriou:2008rp}
T.~P.~Sotiriou and V.~Faraoni,
%``f(R) Theories Of Gravity,''
Rev. Mod. Phys. \textbf{82}, 451-497 (2010)
doi:10.1103/RevModPhys.82.451
[arXiv:0805.1726 [gr-qc]].
%3202 citations counted in INSPIRE as of 18 Jul 2022



%%%%%%%%%%% f(T) %%%%%%%%%%%%%%%%%%%%%%%%%%



%\cite{}
\bibitem{Cai:2015emx}
Y.~F.~Cai, S.~Capozziello, M.~De Laurentis and E.~N.~Saridakis,
%``f(T) teleparallel gravity and cosmology,''
Rept. Prog. Phys. \textbf{79}, no.10, 106901 (2016)
doi:10.1088/0034-4885/79/10/106901
[arXiv:1511.07586 [gr-qc]].
%740 citations counted in INSPIRE as of 18 Jul 2022


%\cite{}
\bibitem{Bahamonde:2021gfp}
S.~Bahamonde, K.~F.~Dialektopoulos, C.~Escamilla-Rivera, G.~Farrugia, V.~Gakis, M.~Hendry, M.~Hohmann, J.~L.~Said, J.~Mifsud and E.~Di Valentino,
%``Teleparallel Gravity: From Theory to Cosmology,''
[arXiv:2106.13793 [gr-qc]].
%85 citations counted in INSPIRE as of 18 Jul 2022


\bibitem{fT1} K. Bamba, R. Myrzakulov, S. Nojiri, S. D. Odintsov, %Reconstruction of f(T) gravity: Rip cosmology,
%finite-time future singularities and thermodynamics, 
Physical Review D 85, 104036 (2012).

\bibitem{fT12} K. Bamba, S. Capozziello, S. Nojiri, S. D. Odintsov, 
%Dark energy cosmology: the equivalent description via different theoretical models and cosmography tests, 
Astrophysics and Space Science (2012) 342:155-228.

\bibitem{fT13} K. Bamba, S. D. Odintsov, D. Saez-Gomez, 
%Conformal symmetry and accelerating cosmology in teleparallelgravity, 
Physical Review D 88, 084042 (2013).






\bibitem{fT41} D.~Momeni, P.~H.~R.~S.~Moraes and R.~Myrzakulov,
%``Generalized second law of thermodynamics in f(R,T) theory of gravity,''
Astrophys. Space Sci. \textbf{361}, no.7, 228 (2016).
%doi:10.1007/s10509-016-2784-2
%[arXiv:1512.04755 [gr-qc]].

\bibitem{fT42} D.~Momeni and R.~Myrzakulov,
%``Conformal Invariant Teleparallel Cosmology,''
Eur. Phys. J. Plus \textbf{129}, 137 (2014).
%doi:10.1140/epjp/i2014-14137-8
%[arXiv:1404.0778 [gr-qc]].

\bibitem{SariRep} Y.~F.~Cai, S.~Capozziello, M.~De Laurentis and E.~N.~Saridakis,
%``f(T) teleparallel gravity and cosmology,''
Rept. Prog. Phys. \textbf{79} (2016) no.10, 106901.


\bibitem{mioultimo}
A.~Casalino, B.~Sanna, L.~Sebastiani and S.~Zerbini,
%``Bounce Models within Teleparallel modified gravity,''
Phys. Rev. D \textbf{103} (2021) no.2, 023514
doi:10.1103/PhysRevD.103.023514
[arXiv:2010.07609 [gr-qc]].





%%%%%%%%%%% f(Q) %%%%%%%%%%%%%%%%%%%%%%%%%%



%\cite{}
\bibitem{Zhao:2021zab}
D.~Zhao,
%``Covariant formulation of f(Q) theory,''
Eur. Phys. J. C \textbf{82}, no.4, 303 (2022)
doi:10.1140/epjc/s10052-022-10266-4
[arXiv:2104.02483 [gr-qc]].
%20 citations counted in INSPIRE as of 18 Jul 2022


%\cite{}
\bibitem{Lazkoz:2019sjl}
R.~Lazkoz, F.~S.~N.~Lobo, M.~Ortiz-Ba\~nos and V.~Salzano,
%``Observational constraints of $f(Q)$ gravity,''
Phys. Rev. D \textbf{100}, no.10, 104027 (2019)
doi:10.1103/PhysRevD.100.104027
[arXiv:1907.13219 [gr-qc]].
%75 citations counted in INSPIRE as of 18 Jul 2022

%\cite{}
\bibitem{Mandal:2020lyq}
S.~Mandal, P.~K.~Sahoo and J.~R.~L.~Santos,
%``Energy conditions in $f(Q)$ gravity,''
Phys. Rev. D \textbf{102}, no.2, 024057 (2020)
doi:10.1103/PhysRevD.102.024057
[arXiv:2008.01563 [gr-qc]].
%58 citations counted in INSPIRE as of 18 Jul 2022

\bibitem{Mandal}
S.~Mandal, A.~Parida and P.~K.~Sahoo,
%``Observational Constraints and Some Toy Models in f(Q) Gravity with Bulk Viscous Fluid,''
Universe \textbf{8} (2022) no.4, 240
doi:10.3390/universe8040240
[arXiv:2103.00171 [gr-qc]].


%\cite{}
\bibitem{Capozziello:2022tvv}
S.~Capozziello and M.~Shokri,
%``Slow-roll inflation in $f (Q)$ non-metric gravity,''
Phys. Dark Univ. \textbf{37} (2022), 101113
%doi:10.1016/j.dark.2022.101113
%[arXiv:2209.06670 [gr-qc]].
%1 citations counted in INSPIRE as of 30 Sep 2022

\bibitem{Hu:2022anq}
K.~Hu, T.~Katsuragawa and T.~Qiu,
%``ADM formulation and Hamiltonian analysis of f(Q) gravity,''
Phys. Rev. D \textbf{106}, no.4, 044025 (2022)
%doi:10.1103/PhysRevD.106.044025
%[arXiv:2204.12826 [gr-qc]].
%3 citations counted in INSPIRE as of 06 Sep 2022

%%%%%%%%%%%%%%%%%%% strong field experiments %%%%%%%%%%%%%%%%%



\bibitem{LIGOScientific:2016aoc}
B.~P.~Abbott \textit{et al.} [LIGO Scientific and Virgo],
%``Observation of Gravitational Waves from a Binary Black Hole Merger,''
Phys. Rev. Lett. \textbf{116}, no.6, 061102 (2016)
%doi:10.1103/PhysRevLett.116.061102
%[arXiv:1602.03837 [gr-qc]].
%8069 citations counted in INSPIRE as of 29 Jun 2022 and the observation of the Black Hole (BH) shadow  the possibility of testing the robustness of GR in highly relativistic regime drive interest  


\bibitem{EventHorizonTelescope:2022xnr}
K.~Akiyama \textit{et al.} [Event Horizon Telescope],
%``First Sagittarius A* Event Horizon Telescope Results. I. The Shadow of the Supermassive Black Hole in the Center of the Milky Way,''
Astrophys. J. Lett. \textbf{930}, no.2, L12 (2022)
%doi:10.3847/2041-8213/ac6674
%51 citations counted in INSPIRE as of 29 Jun 2022


\bibitem{EventHorizonTelescope:2019dse}
K.~Akiyama \textit{et al.} [Event Horizon Telescope],
%``First M87 Event Horizon Telescope Results. I. The Shadow of the Supermassive Black Hole,''
Astrophys. J. Lett. \textbf{875}, L1 (2019)
%doi:10.3847/2041-8213/ab0ec7
%[arXiv:1906.11238 [astro-ph.GA]].
%1669 citations counted in INSPIRE as of 29 Jun 2022 and in the Milky way



\bibitem{Banerjee:2019nnj}
I.~Banerjee, S.~Chakraborty and S.~SenGupta,
%``Silhouette of M87*: A New Window to Peek into the World of Hidden Dimensions,''
Phys. Rev. D \textbf{101}, no.4, 041301 (2020)
%doi:10.1103/PhysRevD.101.041301
%[arXiv:1909.09385 [gr-qc]].
%109 citations counted in INSPIRE as of 29 Jun 2022.


\bibitem{Mark:2017dnq}
Z.~Mark, A.~Zimmerman, S.~M.~Du and Y.~Chen,
%``A recipe for echoes from exotic compact objects,''
Phys. Rev. D \textbf{96}, no.8, 084002 (2017)
%doi:10.1103/PhysRevD.96.084002
%[arXiv:1706.06155 [gr-qc]].
%146 citations counted in INSPIRE as of 29 Jun 2022


\bibitem{Bueno:2017hyj}
P.~Bueno, P.~A.~Cano, F.~Goelen, T.~Hertog and B.~Vercnocke,
%``Echoes of Kerr-like wormholes,''
Phys. Rev. D \textbf{97}, no.2, 024040 (2018)
%doi:10.1103/PhysRevD.97.024040
%[arXiv:1711.00391 [gr-qc]].
%125 citations counted in INSPIRE as of 29 Jun 2022

%%%%%%%%%%%%%%%%%%%%% SSS f(R) %%%%%%%%%%%%%%%%%%

%\cite{}
\bibitem{Multamaki:2006zb}
T.~Multamaki and I.~Vilja,
%``Spherically symmetric solutions of modified field equations in f(R) theories of gravity,''
Phys. Rev. D \textbf{74}, 064022 (2006)
doi:10.1103/PhysRevD.74.064022
[arXiv:astro-ph/0606373 [astro-ph]].
%258 citations counted in INSPIRE as of 18 Jul 2022

%\cite{M}
\bibitem{delaCruz-Dombriz:2009pzc}
A.~de la Cruz-Dombriz, A.~Dobado and A.~L.~Maroto,
%``Black Holes in f(R) theories,''
Phys. Rev. D \textbf{80}, 124011 (2009)
[erratum: Phys. Rev. D \textbf{83}, 029903 (2011)]
doi:10.1103/PhysRevD.80.124011
[arXiv:0907.3872 [gr-qc]].
%206 citations counted in INSPIRE as of 18 Jul 2022

%\cite{}
\bibitem{Kobayashi:2008tq}
T.~Kobayashi and K.~i.~Maeda,
%``Relativistic stars in f(R) gravity, and absence thereof,''
Phys. Rev. D \textbf{78}, 064019 (2008)
doi:10.1103/PhysRevD.78.064019
[arXiv:0807.2503 [astro-ph]].
%149 citations counted in INSPIRE as of 18 Jul 2022


%\cite{}
\bibitem{Upadhye:2009kt}
A.~Upadhye and W.~Hu,
%``The existence of relativistic stars in f(R) gravity,''
Phys. Rev. D \textbf{80}, 064002 (2009)
doi:10.1103/PhysRevD.80.064002
[arXiv:0905.4055 [astro-ph.CO]].
%88 citations counted in INSPIRE as of 18 Jul 2022

%\cite{}
\bibitem{Calza:2018ohl}
M.~Calz\`a, M.~Rinaldi and L.~Sebastiani,
%``A special class of solutions in $F(R)$-gravity,''
Eur. Phys. J. C \textbf{78}, no.3, 178 (2018)
doi:10.1140/epjc/s10052-018-5681-8
[arXiv:1802.00329 [gr-qc]].
%25 citations counted in INSPIRE as of 18 Jul 2022




%%%%%%%%%%%%%%%%%%%%% SSS f(T) %%%%%%%%%%%%%%%%%%



%\cite{}
\bibitem{Aftergood:2014wla}
J.~Aftergood and A.~DeBenedictis,
%``Matter conditions for regular black holes in $f(T)$ gravity,''
Phys. Rev. D \textbf{90}, no.12, 124006 (2014)
doi:10.1103/PhysRevD.90.124006
[arXiv:1409.4084 [gr-qc]].
%26 citations counted in INSPIRE as of 18 Jul 2022


%\cite{}
\bibitem{Bahamonde:2019jkf}
S.~Bahamonde and U.~Camci,
%``Exact Spherically Symmetric Solutions in Modified Teleparallel gravity,''
Symmetry \textbf{11}, no.12, 1462 (2019)
doi:10.3390/sym11121462
[arXiv:1911.03965 [gr-qc]].
%25 citations counted in INSPIRE as of 18 Jul 2022


%
\bibitem{Ilijic:2018ulf}
S.~Ilijic and M.~Sossich,
%``Compact stars in $f(T)$ extended theory of gravity,''
Phys. Rev. D \textbf{98}, no.6, 064047 (2018)
doi:10.1103/PhysRevD.98.064047
[arXiv:1807.03068 [gr-qc]].
%23 citations counted in INSPIRE as of 18 Jul 2022


%\cite{}
\bibitem{LinfT}
R.~h.~Lin, X.~h.~Zhai and X.~z.~Li,
%``Spherical collapse and virialization in $f(T)$ gravities,''
JCAP \textbf{03}, 040 (2017)
doi:10.1088/1475-7516/2017/03/040
[arXiv:1612.05866 [gr-qc]].
%8 citations counted in INSPIRE as of 18 Jul 2022



%\cite{}
\bibitem{DeBenedictis:2016aze}
A.~DeBenedictis and S.~Ilijic,
%``Spherically symmetric vacuum in covariant $F(T) = T + \frac{\alpha}{2}T^{2} + \mathcal{O}(T^{\gamma})$ gravity theory,''
Phys. Rev. D \textbf{94}, no.12, 124025 (2016)
doi:10.1103/PhysRevD.94.124025
[arXiv:1609.07465 [gr-qc]].
%37 citations counted in INSPIRE as of 18 Jul 2022



%%%%%%%%%%%%%%%%%%%%% SSS f(Q) %%%%%%%%%%%%%%%%%%



%\cite{}
\bibitem{Lin}
R.~H.~Lin and X.~H.~Zhai,
%``Spherically symmetric configuration in $f(Q)$ gravity,''
Phys. Rev. D \textbf{103}, no.12, 124001 (2021)
%doi:10.1103/PhysRevD.103.124001
%[arXiv:2105.01484 [gr-qc]].
%23 citations counted in INSPIRE as of 18 Jul 2022

%
\bibitem{Hassan:2022jgn}
Z.~Hassan, G.~Mustafa, J.~R.~L.~Santos and P.~K.~Sahoo,
%``Embedding procedure and wormhole solutions in $f(Q)$ gravity,''
doi:10.1209/0295-5075/ac8017
[arXiv:2207.05304 [gr-qc]].
%0 citations counted in INSPIRE as of 18 Jul 2022

%\cite{}
\bibitem{Tayde:2022lxd}
M.~Tayde, Z.~Hassan, P.~K.~Sahoo and S.~Gutti,
%``Static spherically symmetric wormholes in $f(Q,T)$ gravity,''
doi:10.1088/1674-1137/ac7f22
[arXiv:2206.01184 [gr-qc]].
%0 citations counted in INSPIRE as of 18 Jul 2022

%\cite{}
\bibitem{Sokoliuk:2022efj}
O.~Sokoliuk, Z.~Hassan, P.~K.~Sahoo and A.~Baransky,
%``Traversable wormholes with charge and non-commutative geometry in the $f(Q)$ gravity,''
Annals Phys. \textbf{443}, 168968 (2022)
%doi:10.1016/j.aop.2022.168968
%[arXiv:2201.00743 [gr-qc]].
%1 citations counted in INSPIRE as of 10 Aug 2022


%\cite{}
\bibitem{Banerjee:2021mqk}
A.~Banerjee, A.~Pradhan, T.~Tangphati and F.~Rahaman,
%``Wormhole geometries in $f(Q)$ gravity and the energy conditions,''
Eur. Phys. J. C \textbf{81}, no.11, 1031 (2021)
%doi:10.1140/epjc/s10052-021-09854-7
%[arXiv:2109.15105 [gr-qc]].
%11 citations counted in INSPIRE as of 10 Aug 2022

%\cite{}
\bibitem{Hassan:2022hcb}
Z.~Hassan, S.~Ghosh, P.~K.~Sahoo and K.~Bamba,
%``Casimir Wormholes in Modified Symmetric Teleparallel Gravity,''
[arXiv:2207.09945 [gr-qc]].
%0 citations counted in INSPIRE as of 10 Aug 2022

%\cite{}
\bibitem{Maurya:2022wwa}
S.~K.~Maurya, K.~Newton Singh, S.~V.~Lohakare and B.~Mishra,
%``Anisotropic Strange Star Model Beyond Standard Maximum Mass Limit by Gravitational Decoupling in $f(Q)$ Gravity,''
[arXiv:2208.04735 [gr-qc]].
%0 citations counted in INSPIRE as of 10 Aug 2022

%\cite{}
\bibitem{Parsaei:2022wnu}
F.~Parsaei, S.~Rastgoo and P.~K.~Sahoo,
%``Wormhole in $f(Q)$ gravity,''
[arXiv:2203.06374 [gr-qc]].
%0 citations counted in INSPIRE as of 10 Aug 2022

%\cite{}
\bibitem{Wang:2021zaz}
W.~Wang, H.~Chen and T.~Katsuragawa,
%``Static and spherically symmetric solutions in f(Q) gravity,''
Phys. Rev. D \textbf{105}, no.2, 024060 (2022)
%doi:10.1103/PhysRevD.105.024060
%[arXiv:2110.13565 [gr-qc]].
%11 citations counted in INSPIRE as of 10 Aug 2022

%\cite{}
\bibitem{Mandal:2021qhx}
S.~Mandal, G.~Mustafa, Z.~Hassan and P.~K.~Sahoo,
%``A study of anisotropic spheres in f(Q) gravity with quintessence field,''
Phys. Dark Univ. \textbf{35}, 100934 (2022)
%doi:10.1016/j.dark.2021.100934
%[arXiv:2112.07350 [physics.gen-ph]].
%7 citations counted in INSPIRE as of 10 Aug 2022


%\cite{}
\bibitem{DAmbrosio:2021zpm}
F.~D'Ambrosio, S.~D.~B.~Fell, L.~Heisenberg and S.~Kuhn,
%``Black holes in f(Q) gravity,''
Phys. Rev. D \textbf{105}, no.2, 024042 (2022)
%doi:10.1103/PhysRevD.105.024042
%[arXiv:2109.03174 [gr-qc]].
%25 citations counted in INSPIRE as of 10 Aug 2022

%\cite{}
\bibitem{Bahamonde:2022esv}
S.~Bahamonde, J.~Gigante Valcarcel, L.~J\"arv and J.~Lember,
%``Black hole solutions in scalar-tensor symmetric teleparallel gravity,''
JCAP \textbf{08}, 082 (2022)
%doi:10.1088/1475-7516/2022/08/082
%[arXiv:2206.02725 [gr-qc]].
%1 citations counted in INSPIRE as of 06 Sep 2022

%\cite{}
\bibitem{Bahamonde:2022zgj}
S.~Bahamonde and L.~J\"arv,
%``Coincident gauge for static spherical field configurations in symmetric teleparallel gravity,''
[arXiv:2208.01872 [gr-qc]].
%0 citations counted in INSPIRE as of 06 Sep 2022




%%%%DM
\bibitem{DM1}
P. Salucci, IAU Symp. 244, 53 (2008).
\bibitem{DM2}
L.S. Sparke, J.S. Gallagher, ``Galaxies in the Universe,'' Cambridge University Press, (2007).

%%%Bh bounce
\bibitem{BB} A. Simpson and M. Visser, JCAP 02 (2019), 042;
\bibitem{BB2} A. Simpson, P. Martin-Moruno and M. Visser, Class. Quant. Grav. 36 (2019) no.14, 145007;
\bibitem{BB3} F. S. N. Lobo, M. E. Rodrigues, M. V. d. S. Silva, A. Simpson and M. Visser, Phys. Rev. D 103 (2021) no.8, 084052.
\bibitem{BB4}M.~Calz\'a, [arXiv:2207.10467 [gr-qc]], (2022).

\bibitem{Zerg}
L.~Sebastiani and S.~Zerbini,
``Some remarks on non-singular spherically symmetric space-times,''
[arXiv:2206.03814 [gr-qc]].


%%%WH

\bibitem{Morris}
M.~S.~Morris and K.~S.~Thorne,
%``Wormholes in space-time and their use for interstellar travel: A tool for teaching general relativity,''
Am. J. Phys. \textbf{56} (1988), 395-412.

\bibitem{WH}
L. Flamm, Physikalische Zeitschrift 17, 48 (1916).
\bibitem{WH2}
A. Einstein and N. Rosen, Phys. Rev. 48, 73 (1935).
\bibitem{WH3}
 M. S. Morris and K. S. Thorne, Am. J. Phys. 56, 395 (1988).
 \bibitem{WH4}
 M. S. Morris, K. S. Thorne and U. Yurtsever, Phys. Rev. Lett. 61, 1446 (1988).
 \bibitem{WH5}
M. Visser, ``Lorentzian wormholes: From Einstein to Hawking,'' Woodbury, USA: AIP (1995) 412 p.
\bibitem{WH6}
 J. P. S. Lemos, F. S. N. Lobo and S. Quinet de Oliveira, Phys. Rev. D 68, 064004 (2003).
 \bibitem{WH7}
 F. S. N. Lobo and M. A. Oliveira, Phys. Rev. D 80, 104012 (2009).
 \bibitem{WH8}
K. A. Bronnikov, M. V. Skvortsova and A. A. Starobinsky, Grav. Cosmol. 16,
216 (2010).
\bibitem{WH9}
 F. Duplessis and D. A. Easson, Phys. Rev. D 92, no. 4, 043516 (2015).
 \bibitem{WH10}
 F. S. N. Lobo, Int. J. Mod. Phys. D 25, no. 07, 1630017 (2016).
 \bibitem{WH11}
 F. S. N. Lobo, Fundam. Theor. Phys. 189, pp. (2017).

\bibitem{WHMG}
F. S. N. Lobo and M. A. Oliveira, Phys. Rev. D 80, 104012 (2009).
\bibitem{WHMG2}
K. A. Bronnikov, M. V. Skvortsova and A. A. Starobinsky, Grav. Cosmol. 16,
216 (2010).
\bibitem{WHMG3}
F. Duplessis and D. A. Easson, Phys. Rev. D 92, no. 4, 043516 (2015).

\bibitem{WHMG4}
R. Di Criscienzo, R. Myrzakulov and L. Sebastiani, Class. Quant. Grav. 30, 235013 (2013).


%%%WHcond
\bibitem{WHcond}
M. Visser and D. Hochberg, Annals Israel Phys. Soc. 13, 249 (1997).
\bibitem{WHcond2}
D. Hochberg and M. Visser, Phys. Rev. D 56, 4745 (1997).
\bibitem{WHcond3}
M. Visser, Phys. Rev. D 39, 3182 (1989).



